M$^3$IT: A Large-Scale Dataset towards Multi-Modal Multilingual Instruction Tuning

Instruction tuning has significantly advanced large language models (LLMs) such as ChatGPT, enabling them to align with human instructions across diverse tasks. However, progress in open vision-language models (VLMs) has been limited due to the scarcity of high-quality instruction datasets. To tackle this challenge and promote research in the vision-language field, we introduce the Multi-Modal, Multilingual Instruction Tuning (M$^3$IT) dataset, designed to optimize VLM alignment with human instructions. Our M$^3$IT dataset comprises 40 carefully curated datasets, including 2.4 million instances and 400 manually written task instructions, reformatted into a vision-to-text structure. Key tasks are translated into 80 languages with an advanced translation system, ensuring broader accessibility. M$^3$IT surpasses previous datasets regarding task coverage, instruction number and instance scale. Moreover, we develop Ying-VLM, a VLM model trained on our M$^3$IT dataset, showcasing its potential to answer complex questions requiring world knowledge, generalize to unseen video tasks, and comprehend unseen instructions in Chinese. We have open-sourced the dataset to encourage further research.

==> tables/instructions_stat.tex <==
%\begin{wraptable}{r}{80mm}

\begin{wraptable}[12]{r}{0.5\textwidth}
% \begin{table}[htb!]
    \centering
    \caption{The statistics of our instructions.}
    \small 
    \vskip 0.1in
    \begin{adjustbox}{max width=0.5\textwidth}
    \begin{tabular}{lr}
    \toprule
    Number of different instructions & 400 \\
    \quad - Image Captioning & 52 \\
    \quad - Classification & 113 \\
    \quad - Visual Question Answering & 95 \\
    \quad - Knowledgeable Visual QA & 40 \\
    \quad - Reasoning & 60 \\
    \quad - Generation & 40 \\
    \midrule
    Tokens per instruction & $24.4\pm9.6$  \\
    \midrule
    Instruction edit distance among the same task & $76.6\pm37.2$ \\
    \midrule
    Instruction edit distance across tasks & $106.6\pm39.5$ \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \label{tab:instruct_stat}
% \end{table}
\end{wraptable}

==> tables/main_ret.tex <==
\begin{table}[ht]
  \centering
  \caption{Experiment result of zero-shot video generalization language tasks.}
  \centering
  \begin{tabular}{c|ccc}
    \toprule
    Model & Video Captioning & Video Question Answer & Video Action Classification \\ 
    \midrule
    Ours & & \\
    MiniGPT4 & & \\
    InstructBLIP  & & \\
    \bottomrule
  \end{tabular}
  \label{tab:main_result}
\end{table}

==> tables/ood_ret.tex <==
% \begin{table}[t!]
%   \caption{Experiment result on knowledgeable visual question answering benchmarks. Our Ying-VLM outperforms all the baseline models with consistently better ROUGE-L scores.}
%   \centering
%   \small 
%   \begin{tabular}{lccc}
%     \toprule
%     Model &  OK-VQA & A-OKVQA & ViQuAE  \\ 
%     \midrule
%     BLIP2-Flan-T5-XXL & 9.1  & 15.6  & 9.7  \\ 
%     MiniGPT4 & 23.3   & 21.8 & 24.4 \\
%     InstructBLIP  & 7.1   & 5.9  & 7.3  \\
%     Ying-VLM (Ours) & \textbf{27.5}  & \textbf{24.5}  & \textbf{29.6}  \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:kvqa_ret}
% \end{table}



% \begin{figure}[htbp]
%   \centering
%   \begin{minipage}[b]{0.49\textwidth}
%     \caption{Experiment results on KVQA benchmarks. Our Ying-VLM outperforms all the baseline models with consistently better ROUGE-L scores.}
%     \centering
%     \begin{adjustbox}{max width=\textwidth}
%   \begin{tabular}{lccc}
%     \toprule
%     Model &  OK-VQA & A-OKVQA & ViQuAE  \\ 
%     \midrule
%     BLIP2-Flan-T5-XXL & 9.1  & 15.6  & 9.7  \\ 
%     MiniGPT4 & 23.3   & 21.8 & 24.4 \\
%     InstructBLIP  & 7.1   & 5.9  & 7.3  \\
%     Ying-VLM (Ours) & \textbf{27.5}  & \textbf{24.5}  & \textbf{29.6}  \\
%     \bottomrule
%   \end{tabular}
%   \end{adjustbox}
%     \label{tab:kvqa_ret}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\textwidth}
%     \centering
% \includegraphics[width=\linewidth]{nips23/images/response-comparev2.pdf}
%     \caption{Evaluation results using GPT-4 as an evaluator. Our model outperforms MiniGPT-4 and InstructBLIP with winning rate at 55.6\% and 65.5\%, respectively.}
%     \label{fig:gpt-4-eval}
%   \end{minipage}
% \end{figure}

